Optimizing Automatic Differentiation with Deep Reinforcement Learning

Computing Jacobians with automatic differentiation is ubiquitous in many scientific domains such as machine learning, computational fluid dynamics, robotics and finance. Even small savings in the number of computations or memory usage in Jacobian computations can already incur massive savings in energy consumption and runtime. While there exist many methods that allow for such savings, they generally trade computational efficiency for approximations of the exact Jacobian. In this paper, we present a novel method to optimize the number of necessary multiplications for Jacobian computation by leveraging deep reinforcement learning (RL) and a concept called cross-country elimination while still computing the exact Jacobian. Cross-country elimination is a framework for automatic differentiation that phrases Jacobian accumulation as ordered elimination of all vertices on the computational graph where every elimination incurs a certain computational cost. We formulate the search for the optimal elimination order that minimizes the number of necessary multiplications as a single player game which is played by an RL agent. We demonstrate that this method achieves up to 33% improvements over state-of-the-art methods on several relevant tasks taken from diverse domains. Furthermore, we show that these theoretical gains translate into actual runtime improvements by providing a cross-country elimination interpreter in JAX that can efficiently execute the obtained elimination orders.

==> figures/elimination.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,491); %set diagram left start at 0, and has height of 491

%Shape: Circle [id:dp9548018857379407] 
\draw   (140.2,139.5) .. controls (140.2,132.6) and (145.8,127) .. (152.7,127) .. controls (159.6,127) and (165.2,132.6) .. (165.2,139.5) .. controls (165.2,146.4) and (159.6,152) .. (152.7,152) .. controls (145.8,152) and (140.2,146.4) .. (140.2,139.5) -- cycle ;
%Shape: Rectangle [id:dp9172506118934006] 
\draw   (20,45.5) -- (268.67,45.5) -- (268.67,235.75) -- (20,235.75) -- cycle ;
%Shape: Circle [id:dp6441915731641329] 
\draw   (220.07,69.83) .. controls (220.07,62.93) and (225.66,57.33) .. (232.57,57.33) .. controls (239.47,57.33) and (245.07,62.93) .. (245.07,69.83) .. controls (245.07,76.74) and (239.47,82.33) .. (232.57,82.33) .. controls (225.66,82.33) and (220.07,76.74) .. (220.07,69.83) -- cycle ;
%Shape: Circle [id:dp4084356887497679] 
\draw   (220.47,209.23) .. controls (220.47,202.33) and (226.06,196.73) .. (232.97,196.73) .. controls (239.87,196.73) and (245.47,202.33) .. (245.47,209.23) .. controls (245.47,216.14) and (239.87,221.73) .. (232.97,221.73) .. controls (226.06,221.73) and (220.47,216.14) .. (220.47,209.23) -- cycle ;
%Shape: Circle [id:dp45150982716175214] 
\draw   (40.2,139.5) .. controls (40.2,132.6) and (45.8,127) .. (52.7,127) .. controls (59.6,127) and (65.2,132.6) .. (65.2,139.5) .. controls (65.2,146.4) and (59.6,152) .. (52.7,152) .. controls (45.8,152) and (40.2,146.4) .. (40.2,139.5) -- cycle ;
%Shape: Rectangle [id:dp6253083128708061] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] (93.2,131.8) -- (110.6,131.8) -- (110.6,147.4) -- (93.2,147.4) -- cycle ;
%Straight Lines [id:da26621021975413484] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (65.2,139.5) -- (93.4,139.4) ;
%Straight Lines [id:da9766018801422383] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (111,139.8) -- (137.2,139.53) ;
\draw [shift={(140.2,139.5)}, rotate = 179.41] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp5861537382129317] 
\draw   (183.6,165.2) -- (204.6,165.2) -- (204.6,181.4) -- (183.6,181.4) -- cycle ;
%Shape: Rectangle [id:dp5406226621025503] 
\draw   (184.6,95) -- (204.2,95) -- (204.2,111.8) -- (184.6,111.8) -- cycle ;
%Straight Lines [id:da8390820282834278] 
\draw    (162.6,131) -- (184.6,111.8) ;
%Straight Lines [id:da7939014673586693] 
\draw    (183.6,165.2) -- (162.2,148.2) ;
%Straight Lines [id:da8057497941196463] 
\draw    (204.2,95) -- (220.79,79.83) ;
\draw [shift={(223,77.8)}, rotate = 137.54] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da8842143305738487] 
\draw    (204.6,181.4) -- (223.9,197.48) ;
\draw [shift={(226.2,199.4)}, rotate = 219.81] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da5157540223155354] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (52.7,127) .. controls (60.67,109.17) and (75,81.5) .. (102.33,69.83) ;
%Curve Lines [id:da8368690890180173] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (52.7,152) .. controls (60,168.17) and (77.67,198.17) .. (102,209.83) ;
%Curve Lines [id:da19918542741033218] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (178.33,70.33) .. controls (201.26,70.18) and (208.08,70.17) .. (217.12,69.92) ;
\draw [shift={(220.07,69.83)}, rotate = 178.22] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da7081560672916272] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (178.73,209.73) .. controls (201.66,209.58) and (208.48,209.57) .. (217.52,209.32) ;
\draw [shift={(220.47,209.23)}, rotate = 178.22] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Circle [id:dp03154551615594259] 
\draw   (119.2,360.5) .. controls (119.2,353.6) and (124.8,348) .. (131.7,348) .. controls (138.6,348) and (144.2,353.6) .. (144.2,360.5) .. controls (144.2,367.4) and (138.6,373) .. (131.7,373) .. controls (124.8,373) and (119.2,367.4) .. (119.2,360.5) -- cycle ;
%Shape: Rectangle [id:dp6331163434071998] 
\draw   (20,266.5) -- (268.67,266.5) -- (268.67,456.75) -- (20,456.75) -- cycle ;
%Shape: Circle [id:dp3712222217851653] 
\draw   (41.07,290.83) .. controls (41.07,283.93) and (46.66,278.33) .. (53.57,278.33) .. controls (60.47,278.33) and (66.07,283.93) .. (66.07,290.83) .. controls (66.07,297.74) and (60.47,303.33) .. (53.57,303.33) .. controls (46.66,303.33) and (41.07,297.74) .. (41.07,290.83) -- cycle ;
%Shape: Circle [id:dp9217767759114438] 
\draw   (39.47,430.23) .. controls (39.47,423.33) and (45.06,417.73) .. (51.97,417.73) .. controls (58.87,417.73) and (64.47,423.33) .. (64.47,430.23) .. controls (64.47,437.14) and (58.87,442.73) .. (51.97,442.73) .. controls (45.06,442.73) and (39.47,437.14) .. (39.47,430.23) -- cycle ;
%Shape: Circle [id:dp0015861607051540494] 
\draw   (219.7,360.5) .. controls (219.7,353.6) and (225.3,348) .. (232.2,348) .. controls (239.1,348) and (244.7,353.6) .. (244.7,360.5) .. controls (244.7,367.4) and (239.1,373) .. (232.2,373) .. controls (225.3,373) and (219.7,367.4) .. (219.7,360.5) -- cycle ;
%Shape: Rectangle [id:dp03256809178507336] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] (172.2,352.8) -- (189.6,352.8) -- (189.6,368.4) -- (172.2,368.4) -- cycle ;
%Straight Lines [id:da21927616197382216] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (144.2,360.5) -- (172.4,360.4) ;
%Straight Lines [id:da17146589631965115] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (190,360.8) -- (216.2,360.53) ;
\draw [shift={(219.2,360.5)}, rotate = 179.41] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp7242521263759177] 
\draw   (84.6,385.7) -- (105.6,385.7) -- (105.6,401.9) -- (84.6,401.9) -- cycle ;
%Shape: Rectangle [id:dp362806174211708] 
\draw   (84.1,318) -- (103.7,318) -- (103.7,334.8) -- (84.1,334.8) -- cycle ;
%Straight Lines [id:da01817853387730739] 
\draw    (62.5,298.5) -- (84.1,318) ;
%Straight Lines [id:da5243405707930483] 
\draw    (61.5,421.75) -- (84.6,401.9) ;
%Straight Lines [id:da1563842322493686] 
\draw    (105.6,385.7) -- (120.8,371.64) ;
\draw [shift={(123,369.6)}, rotate = 137.22] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7207203314608727] 
\draw    (103.7,334.8) -- (120.36,349.61) ;
\draw [shift={(122.6,351.6)}, rotate = 221.63] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da8865247312223875] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (66.07,290.83) -- (109.8,290.4) ;
%Straight Lines [id:da7638230927616959] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (64.47,430.23) -- (110.2,430) ;
%Curve Lines [id:da6842740935273973] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (185.4,290) .. controls (208.2,300.26) and (224.5,328.21) .. (231.22,345.38) ;
\draw [shift={(232.2,348)}, rotate = 250.35] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da22339675209691] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (187,429.6) .. controls (222.72,411.36) and (226.31,393.84) .. (231.38,375.85) ;
\draw [shift={(232.2,373)}, rotate = 106.42] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Circle [id:dp32626497479379246] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (413.87,139.5) .. controls (413.87,132.6) and (419.46,127) .. (426.37,127) .. controls (433.27,127) and (438.87,132.6) .. (438.87,139.5) .. controls (438.87,146.4) and (433.27,152) .. (426.37,152) .. controls (419.46,152) and (413.87,146.4) .. (413.87,139.5) -- cycle ;
%Shape: Rectangle [id:dp5853598562858913] 
\draw   (302.67,45.5) -- (551.33,45.5) -- (551.33,455.73) -- (302.67,455.73) -- cycle ;
%Shape: Circle [id:dp26782892097996946] 
\draw   (471.4,91.17) .. controls (471.4,84.26) and (477,78.67) .. (483.9,78.67) .. controls (490.8,78.67) and (496.4,84.26) .. (496.4,91.17) .. controls (496.4,98.07) and (490.8,103.67) .. (483.9,103.67) .. controls (477,103.67) and (471.4,98.07) .. (471.4,91.17) -- cycle ;
%Shape: Circle [id:dp05594306106928837] 
\draw   (470.13,187.9) .. controls (470.13,181) and (475.73,175.4) .. (482.63,175.4) .. controls (489.54,175.4) and (495.13,181) .. (495.13,187.9) .. controls (495.13,194.8) and (489.54,200.4) .. (482.63,200.4) .. controls (475.73,200.4) and (470.13,194.8) .. (470.13,187.9) -- cycle ;
%Straight Lines [id:da9636978624323339] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (436.33,131.73) -- (471.41,101.04) ;
\draw [shift={(473.67,99.07)}, rotate = 138.81] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da6100044005076131] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (436.33,147.73) -- (469.77,177.73) ;
\draw [shift={(472,179.73)}, rotate = 221.9] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Circle [id:dp7203788215347473] 
\draw   (356.73,92.17) .. controls (356.73,85.26) and (362.33,79.67) .. (369.23,79.67) .. controls (376.14,79.67) and (381.73,85.26) .. (381.73,92.17) .. controls (381.73,99.07) and (376.14,104.67) .. (369.23,104.67) .. controls (362.33,104.67) and (356.73,99.07) .. (356.73,92.17) -- cycle ;
%Straight Lines [id:da0795125134666772] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (379.67,99.73) -- (413.4,129.1) ;
\draw [shift={(415.67,131.07)}, rotate = 221.04] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Circle [id:dp5835058998061966] 
\draw   (357.07,189.5) .. controls (357.07,182.6) and (362.66,177) .. (369.57,177) .. controls (376.47,177) and (382.07,182.6) .. (382.07,189.5) .. controls (382.07,196.4) and (376.47,202) .. (369.57,202) .. controls (362.66,202) and (357.07,196.4) .. (357.07,189.5) -- cycle ;
%Straight Lines [id:da7975912056836592] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ]   (379.67,180.4) -- (414.09,149.73) ;
\draw [shift={(416.33,147.73)}, rotate = 138.3] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Circle [id:dp14537073648608745] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (415.2,344.17) .. controls (415.2,337.26) and (420.8,331.67) .. (427.7,331.67) .. controls (434.6,331.67) and (440.2,337.26) .. (440.2,344.17) .. controls (440.2,351.07) and (434.6,356.67) .. (427.7,356.67) .. controls (420.8,356.67) and (415.2,351.07) .. (415.2,344.17) -- cycle ;
%Shape: Circle [id:dp01909654238583014] 
\draw   (472.73,295.83) .. controls (472.73,288.93) and (478.33,283.33) .. (485.23,283.33) .. controls (492.14,283.33) and (497.73,288.93) .. (497.73,295.83) .. controls (497.73,302.74) and (492.14,308.33) .. (485.23,308.33) .. controls (478.33,308.33) and (472.73,302.74) .. (472.73,295.83) -- cycle ;
%Shape: Circle [id:dp7452468085929822] 
\draw   (471.47,392.57) .. controls (471.47,385.66) and (477.06,380.07) .. (483.97,380.07) .. controls (490.87,380.07) and (496.47,385.66) .. (496.47,392.57) .. controls (496.47,399.47) and (490.87,405.07) .. (483.97,405.07) .. controls (477.06,405.07) and (471.47,399.47) .. (471.47,392.57) -- cycle ;
%Shape: Circle [id:dp39410233433804354] 
\draw   (358.07,296.83) .. controls (358.07,289.93) and (363.66,284.33) .. (370.57,284.33) .. controls (377.47,284.33) and (383.07,289.93) .. (383.07,296.83) .. controls (383.07,303.74) and (377.47,309.33) .. (370.57,309.33) .. controls (363.66,309.33) and (358.07,303.74) .. (358.07,296.83) -- cycle ;
%Shape: Circle [id:dp7371562793598473] 
\draw   (358.4,394.17) .. controls (358.4,387.26) and (364,381.67) .. (370.9,381.67) .. controls (377.8,381.67) and (383.4,387.26) .. (383.4,394.17) .. controls (383.4,401.07) and (377.8,406.67) .. (370.9,406.67) .. controls (364,406.67) and (358.4,401.07) .. (358.4,394.17) -- cycle ;
%Straight Lines [id:da8718463737625154] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (383.07,296.83) -- (469.73,295.87) ;
\draw [shift={(472.73,295.83)}, rotate = 179.36] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da616954204108357] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (383.4,394.17) -- (468.47,392.62) ;
\draw [shift={(471.47,392.57)}, rotate = 178.96] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da7065882139795215] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (383.07,296.83) .. controls (432.15,305.47) and (471.88,348.38) .. (483.02,377.41) ;
\draw [shift={(483.97,380.07)}, rotate = 251.62] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da8979260896607746] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (383.4,394.17) .. controls (432.74,402.84) and (473.58,343.49) .. (484.46,310.79) ;
\draw [shift={(485.23,308.33)}, rotate = 106.61] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da3124824485054748] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=0.75 ][line width=4.5]    (412.37,329.83) -- (443.03,358.5) ;
%Straight Lines [id:da28738565789738124] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=0.75 ][line width=4.5]    (414,357.73) -- (441.67,330.73) ;

% Text Node
\draw (46,130.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{i}$};
% Text Node
\draw (145.4,129.8) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{j}$};
% Text Node
\draw (222.6,58.6) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k_{1}}$};
% Text Node
\draw (222.8,199.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k_{n}}$};
% Text Node
\draw (94.4,130.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$c_{ij}$};
% Text Node
\draw    (103,58.4) -- (178,58.4) -- (178,81.4) -- (103,81.4) -- cycle  ;
\draw (106,62.8) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$c_{ik_{1}} +\ c_{ij} c_{jk_{1}}$};
% Text Node
\draw    (102.93,197.93) -- (178.93,197.93) -- (178.93,220.93) -- (102.93,220.93) -- cycle  ;
\draw (105.93,202.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$c_{ik_{n}} +\ c_{ij} c_{jk_{n}}$};
% Text Node
\draw (184.8,93.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$c_{jk_{1}}$};
% Text Node
\draw (184.8,163.8) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$c_{jk_{n}}$};
% Text Node
\draw    (20,20.5) -- (137,20.5) -- (137,45.5) -- (20,45.5) -- cycle  ;
\draw (23,24.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {Front Elimination};
% Text Node
\draw (224.5,351.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k}$};
% Text Node
\draw (124.4,350.8) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{j}$};
% Text Node
\draw (43.6,280.6) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{i_{1}}$};
% Text Node
\draw (41.8,420.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{i_{n}}$};
% Text Node
\draw (173.4,351.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$c_{jk}$};
% Text Node
\draw    (110,277.9) -- (185,277.9) -- (185,300.9) -- (110,300.9) -- cycle  ;
\draw (113,282.3) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$c_{i_{1} k} +\ c_{i_{1} j} c_{j k}$};
% Text Node
\draw    (110.43,417.43) -- (186.43,417.43) -- (186.43,440.43) -- (110.43,440.43) -- cycle  ;
\draw (113.43,421.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$c_{i_{n} k} +\ c_{i_{n} j} c_{jk}$};
% Text Node
\draw (84.3,316.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$c_{i_{1} j}$};
% Text Node
\draw (84.8,384.3) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize]  {$c_{i_{n} j}$};
% Text Node
\draw    (20,241.5) -- (136,241.5) -- (136,266.5) -- (20,266.5) -- cycle  ;
\draw (23,245.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {Back Elimination};
% Text Node
\draw (419.07,129.8) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$v_{j}$};
% Text Node
\draw (473.93,79.93) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k_{1}}$};
% Text Node
\draw (472.47,178.07) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k_{n}}$};
% Text Node
\draw    (302.67,20.5) -- (425.67,20.5) -- (425.67,45.5) -- (302.67,45.5) -- cycle  ;
\draw (305.67,24.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {Vertex Elimination};
% Text Node
\draw (359.27,80.93) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k_{1}}$};
% Text Node
\draw (359.6,178.27) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k_{1}}$};
% Text Node
\draw (395.31,93.49) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=-41.81] [align=left] {front};
% Text Node
\draw (376.03,164.02) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=-317.36] [align=left] {front};
% Text Node
\draw (433.16,115.21) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=-320.67] [align=left] {back};
% Text Node
\draw (448.64,139.87) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=-41.67] [align=left] {back};
% Text Node
\draw (420.4,334.47) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$v_{j}$};
% Text Node
\draw (475.27,284.6) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k_{1}}$};
% Text Node
\draw (473.8,382.73) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k_{n}}$};
% Text Node
\draw (360.6,285.6) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k_{1}}$};
% Text Node
\draw (360.93,382.93) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$v_{k_{1}}$};


\end{tikzpicture}


==> figures/graph_repr.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,452); %set diagram left start at 0, and has height of 452

%Flowchart: Connector [id:dp6479817213194753] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.38 ][line width=0.75]  (391,48) .. controls (391,38.61) and (398.61,31) .. (408,31) .. controls (417.39,31) and (425,38.61) .. (425,48) .. controls (425,57.39) and (417.39,65) .. (408,65) .. controls (398.61,65) and (391,57.39) .. (391,48) -- cycle ;
%Flowchart: Connector [id:dp9479463396577028] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.38 ][line width=0.75]  (621,48) .. controls (621,38.61) and (628.61,31) .. (638,31) .. controls (647.39,31) and (655,38.61) .. (655,48) .. controls (655,57.39) and (647.39,65) .. (638,65) .. controls (628.61,65) and (621,57.39) .. (621,48) -- cycle ;
%Flowchart: Connector [id:dp8811146151512207] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.38 ][line width=0.75]  (509,152) .. controls (509,142.61) and (516.61,135) .. (526,135) .. controls (535.39,135) and (543,142.61) .. (543,152) .. controls (543,161.39) and (535.39,169) .. (526,169) .. controls (516.61,169) and (509,161.39) .. (509,152) -- cycle ;
%Flowchart: Connector [id:dp5724290557814014] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.38 ][line width=0.75]  (509,291) .. controls (509,281.61) and (516.61,274) .. (526,274) .. controls (535.39,274) and (543,281.61) .. (543,291) .. controls (543,300.39) and (535.39,308) .. (526,308) .. controls (516.61,308) and (509,300.39) .. (509,291) -- cycle ;
%Flowchart: Connector [id:dp09800527223228561] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ][line width=0.75]  (631,405) .. controls (631,395.61) and (638.61,388) .. (648,388) .. controls (657.39,388) and (665,395.61) .. (665,405) .. controls (665,414.39) and (657.39,422) .. (648,422) .. controls (638.61,422) and (631,414.39) .. (631,405) -- cycle ;
%Flowchart: Connector [id:dp17156888332719866] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ][line width=0.75]  (391,405) .. controls (391,395.61) and (398.61,388) .. (408,388) .. controls (417.39,388) and (425,395.61) .. (425,405) .. controls (425,414.39) and (417.39,422) .. (408,422) .. controls (398.61,422) and (391,414.39) .. (391,405) -- cycle ;
%Straight Lines [id:da47806398261046146] 
\draw [line width=1.5]    (526,169) -- (526,185.5) ;
%Straight Lines [id:da2713889570360857] 
\draw [line width=1.5]    (627,59.5) -- (610,77.5) ;
%Straight Lines [id:da1662396114700947] 
\draw [line width=1.5]    (420,60.5) -- (441,80.5) ;
%Straight Lines [id:da4720675750595308] 
\draw [line width=1.5]    (440,371.5) -- (422.76,389.6) ;
\draw [shift={(420,392.5)}, rotate = 313.6] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da7232307716191954] 
\draw [line width=1.5]    (614,369.5) -- (633.3,390.55) ;
\draw [shift={(636,393.5)}, rotate = 227.49] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da08682146176506356] 
\draw [line width=1.5]    (526,231.5) -- (526,270) ;
\draw [shift={(526,274)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da9011682680641069] 
\draw [line width=1.5]    (554,124) -- (541.69,137.54) ;
\draw [shift={(539,140.5)}, rotate = 312.27] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da3664372755664592] 
\draw [line width=1.5]    (498,127) -- (511.04,138.81) ;
\draw [shift={(514,141.5)}, rotate = 222.18] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da3957388307182482] 
\draw [line width=1.5]    (538,303.5) -- (555,322.5) ;
%Straight Lines [id:da44454748713591863] 
\draw [line width=1.5]    (516,305.5) -- (501,323.5) ;
%Straight Lines [id:da4226718097918115] 
\draw [line width=1.5]    (614,332.5) -- (640.21,384.92) ;
\draw [shift={(642,388.5)}, rotate = 243.43] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da9087067815114256] 
\draw [line width=1.5]    (566,232.5) -- (575,251.5) ;
%Straight Lines [id:da5664794096021277] 
\draw [line width=1.5]    (533,166.5) -- (542,184.5) ;
%Straight Lines [id:da46180223324020475] 
\draw [line width=1.5]    (598,299.5) -- (610,323.5) ;
%Shape: Rectangle [id:dp7178085171664923] 
\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.38 ] (59,292.5) -- (182,292.5) -- (182,311.5) -- (59,311.5) -- cycle ;
%Shape: Rectangle [id:dp458202405951027] 
\draw  [draw opacity=0][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.38 ] (92,240.5) -- (114,240.5) -- (114,395) -- (92,395) -- cycle ;
%Shape: Rectangle [id:dp8057339163145304] 
\draw   (52,235) -- (249,235) -- (249,437.5) -- (52,437.5) -- cycle ;

% Text Node
\draw    (51,34.75) -- (344,34.75) -- (344,197.75) -- (51,197.75) -- cycle  ;
\draw (197.5,116.25) node   [align=left] {\begin{minipage}[lt]{196.52pt}\setlength\topsep{0pt}
{\fontfamily{pcr}\selectfont \{ lambda ; \textcolor[rgb]{0.82,0.01,0.11}{a}:f32[] \textcolor[rgb]{0.82,0.01,0.11}{b}:f32[]. let}\\{\fontfamily{pcr}\selectfont 	\textcolor[rgb]{0.29,0.56,0.89}{c}:f32[] = mul \textcolor[rgb]{0.82,0.01,0.11}{a} \textcolor[rgb]{0.82,0.01,0.11}{b}}\\{\fontfamily{pcr}\selectfont 	\textcolor[rgb]{0.29,0.56,0.89}{d}:f32[] = sin \textcolor[rgb]{0.29,0.56,0.89}{c}}\\{\fontfamily{pcr}\selectfont 	\textcolor[rgb]{0.25,0.46,0.02}{e}:f32[] = add \textcolor[rgb]{0.29,0.56,0.89}{d} \textcolor[rgb]{0.29,0.56,0.89}{c}}\\{\fontfamily{pcr}\selectfont 	\textcolor[rgb]{0.25,0.46,0.02}{f}:f32[] = log \textcolor[rgb]{0.29,0.56,0.89}{d}}\\{\fontfamily{pcr}\selectfont  in (\textcolor[rgb]{0.25,0.46,0.02}{e}, \textcolor[rgb]{0.25,0.46,0.02}{f}) \}}
\end{minipage}};
% Text Node
\draw    (440,81) -- (497,81) -- (497,128) -- (440,128) -- cycle  ;
\draw (443,85.4) node [anchor=north west][inner sep=0.75pt]    {$\frac{\partial c}{\partial a} =b$};
% Text Node
\draw (403,37.4) node [anchor=north west][inner sep=0.75pt]    {$a$};
% Text Node
\draw (633,39.4) node [anchor=north west][inner sep=0.75pt]    {$b$};
% Text Node
\draw (521,141.9) node [anchor=north west][inner sep=0.75pt]    {$c$};
% Text Node
\draw (520,282.9) node [anchor=north west][inner sep=0.75pt]    {$d$};
% Text Node
\draw (403,394.9) node [anchor=north west][inner sep=0.75pt]    {$e$};
% Text Node
\draw (642,394.9) node [anchor=north west][inner sep=0.75pt]    {$f$};
% Text Node
\draw    (554,78) -- (611,78) -- (611,125) -- (554,125) -- cycle  ;
\draw (557,82.4) node [anchor=north west][inner sep=0.75pt]    {$\frac{\partial c}{\partial b} =a$};
% Text Node
\draw    (562,252) -- (621,252) -- (621,299) -- (562,299) -- cycle  ;
\draw (565,256.4) node [anchor=north west][inner sep=0.75pt]    {$\frac{\partial f}{\partial c} =1$};
% Text Node
\draw    (484,185) -- (568,185) -- (568,232) -- (484,232) -- cycle  ;
\draw (487,189.4) node [anchor=north west][inner sep=0.75pt]    {$\frac{\partial d}{\partial c} =\cos c$};
% Text Node
\draw    (439,324) -- (501,324) -- (501,371) -- (439,371) -- cycle  ;
\draw (442,328.4) node [anchor=north west][inner sep=0.75pt]    {$\frac{\partial e}{\partial d} =\frac{1}{d}$};
% Text Node
\draw    (555,323) -- (614,323) -- (614,370) -- (555,370) -- cycle  ;
\draw (558,327.4) node [anchor=north west][inner sep=0.75pt]    {$\frac{\partial f}{\partial d} =1$};
% Text Node
\draw (85,248.9) node [anchor=north west][inner sep=0.75pt]    {$\begin{pmatrix}
1 &  &  & \\
1 &  &  & \\
 & 1 &  & \\
 &  & 1 & 1\\
 &  &  & 1\\
 &  &  & 
\end{pmatrix}$};
% Text Node
\draw (65,248.4) node [anchor=north west][inner sep=0.75pt]    {$a$};
% Text Node
\draw (65,270.4) node [anchor=north west][inner sep=0.75pt]    {$b$};
% Text Node
\draw (66,291.4) node [anchor=north west][inner sep=0.75pt]    {$c$};
% Text Node
\draw (66,312.4) node [anchor=north west][inner sep=0.75pt]    {$d$};
% Text Node
\draw (67,334.4) node [anchor=north west][inner sep=0.75pt]    {$e$};
% Text Node
\draw (65,355.4) node [anchor=north west][inner sep=0.75pt]    {$f$};
% Text Node
\draw (98,375.4) node [anchor=north west][inner sep=0.75pt]    {$c$};
% Text Node
\draw (116,375.4) node [anchor=north west][inner sep=0.75pt]    {$d$};
% Text Node
\draw (137,375.4) node [anchor=north west][inner sep=0.75pt]    {$e$};
% Text Node
\draw (154,376.4) node [anchor=north west][inner sep=0.75pt]    {$f$};
% Text Node
\draw (73,394) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{42.84pt}\setlength\topsep{0pt}
\textcolor[rgb]{0.82,0.01,0.11}{incoming}
\begin{center}
\textcolor[rgb]{0.82,0.01,0.11}{edges}
\end{center}

\end{minipage}};
% Text Node
\draw (184,280.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{40.12pt}\setlength\topsep{0pt}
\textcolor[rgb]{0.29,0.56,0.89}{outgoing}
\begin{center}
\textcolor[rgb]{0.29,0.56,0.89}{edges}
\end{center}

\end{minipage}};
% Text Node
\draw    (51,9.5) -- (137,9.5) -- (137,34.5) -- (51,34.5) -- cycle  ;
\draw (54,13.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {Jaxpression};
% Text Node
\draw    (52,209.5) -- (203,209.5) -- (203,234.5) -- (52,234.5) -- cycle  ;
\draw (55,213.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {Graph Representation};


\end{tikzpicture}

